Semantic Image Segmentation with Deep Convolutional Nets and Fully Connected CRFs

Deep Convolutional Neural Networks (DCNNs) have recently shown state of the art performance in high level vision tasks, such as image classification and object detection. This work brings together methods from DCNNs and probabilistic graphical models for addressing the task of pixel-level classification (also called "semantic image segmentation"). We show that responses at the final layer of DCNNs are not sufficiently localized for accurate object segmentation. This is due to the very invariance properties that make DCNNs good for high level tasks. We overcome this poor localization property of deep networks by combining the responses at the final DCNN layer with a fully connected Conditional Random Field (CRF). Qualitatively, our "DeepLab" system is able to localize segment boundaries at a level of accuracy which is beyond previous methods. Quantitatively, our method sets the new state-of-art at the PASCAL VOC-2012 semantic image segmentation task, reaching 71.6% IOU accuracy in the test set. We show how these results can be obtained efficiently: Careful network re-purposing and a novel application of the 'hole' algorithm from the wavelet community allow dense computation of neural net responses at 8 frames per second on a modern GPU.

==> densecrf_detail.tex <==
We briefly review the efficient inference in fully connected CRFs, and refer readers to \citep{krahenbuhl2011efficient} for more details. 

The CRF distribution over pixels is defined as follows.
\begin{align}
  P(\boldsymbol{x}) = \frac{1}{Z} \exp \Big(-E(\boldsymbol{x})\Big)
\end{align}
where $\boldsymbol{x}$ is the label assignment for pixels, and $E(\boldsymbol{x})$ is the energy function. In our experiments, the energy function is
\begin{align}
  E(\boldsymbol{x}) = \sum_i \theta_i(x_i) + \sum_{ij} \theta_{ij}(x_i, x_j)
\end{align}
where the unary potential $\theta_i(x_i) = - \log P(x_i)$, $P(x_i)$ is the probability of assigning label to pixel $i$ (this probability is computed by DCNN), and the pairwise potential $\theta_{ij}(x_i, x_j) = \sum_{m=1}^{K} w^m \cdot k^m(\boldsymbol{f}_i, \boldsymbol{f}_j)$. The edge set is the fully connected edges between any $i$ and $j$, and each $k^m$ is the Gaussian kernel depends on features extracted for piexl $i$ and $j$ and is weighted by parameter $w^m$. We employ the bilateral filtering, which define the kernels as 
\begin{align}
  \theta_{ij}(x_i, x_j) = w^1 \exp \Big(-\frac{|p_i-p_j|^2}{2\sigma_\alpha^2} -\frac{|I_i-I_j|^2}{2\sigma_\beta^2} \Big) + w^2 \exp \Big(-\frac{|p_i-p_j|^2}{2\sigma_\gamma^2}\Big)
\end{align}
where the first kernel depends on both pixel positions (denoted as $p$) and pixel color intensities (denoted as $I$), and the second kernel only depends on pixel positions. The hyper parameters $\sigma_\alpha$, $\sigma_\beta$ and $\sigma_\gamma$ control the ``nearness'' of the Gaussian kernels.

The efficient inference algorithm is based on mean field approximation to the CRF distribution, which finds another simple distribution $b(\boldsymbol{x}) = \prod_i b_i(x_i)$ that minimizes the KL-divergence $KL(b(\boldsymbol{x}) \| P(\boldsymbol{x}))$. The resulting algorithm is stated in \figref{fig:InferenceCRF}. Within the while loop, the first step (\ie, the message passing step) can be expressed as a convolution with a Gaussian kernel in feature space. High-dimensional filtering algorihtms \citep{adams2010fast} have been proposed to speed-up this computation.

\begin{figure}[t]
%\vspace{-0.5cm}
\fbox{
\begin{minipage}[c]{13.5cm}
{\bf Algorithm: Efficient Inference in Fully Connected CRFs}

Initialize $b_i(x_i) \leftarrow \frac{1}{Z_i} \exp \Big(-\theta_i(x_i) \Big)$

{\bf While} not converged, 

\begin{enumerate}[labelindent=0pt,labelwidth=\widthof{\ref{last-item}},label=\arabic*.,itemindent=2em,leftmargin=0pt]
\item $\tilde{b_i}^m(l) \leftarrow \sum_{j \neq i}k^m(\boldsymbol{f}_i,\boldsymbol{f}_j) \cdot b_j(l), \ \forall m$
\item $\hat{b_i}(x_i) \leftarrow \sum_{l} \sum_m w^m \cdot \tilde{b_i}^m(l)$
\item $b_i(x_i) \propto \exp \Big(-\theta_i(x_i) - \hat{b_i}(x_i) \Big)$
\end{enumerate}

\end{minipage}
}
\caption{Efficient Inference algorithm in Fully Connected CRFs
}
\label{fig:InferenceCRF}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> related.tex <==
\subsection{Related Work}
Our model is mostly related to two fields, and the goal of this work is to combine the best from them.

{\bf{Conditional Random Fields for segmentation: }} Many semantic segmentation methods rely on Conditional Random Fields (CRFs), which model the local interactions between pixels \citep{rother2004grabcut, shotton2009textonboost} or superpixels \citep{lucchi2011spatial} via the pairwise potential. Several works have been proposed to model the hierarchical dependency \citep{he2004multiscale, ladicky2009associative, lempitsky2011pylon} and the high-order potential (in addition to pairwise potential) \citep{delong2012fast, gonfaus2010harmony, kohli2009robust, krahenbuhl2011efficient}. Our model takes use of the efficient inference algorithm in fully connected CRF proposed by \citet{krahenbuhl2011efficient} for its powerful long range dependency. Note that mean field had been extensively studied for traditional image segmentation/edge detection tasks citep{geiger1991common, geiger1991parallel, kokkinos2008computational}, but \citet{krahenbuhl2011efficient} showed that it can be very efficient in the context of semantic segmentation.

{\bf{Deep Convolutional Neural Network for segmentation: }} Most of the systems built on top of DCNN classify either a single object label for an entire image \citep{KrizhevskyNIPS2013, simonyan2014very, szegedy2014going}, or several object labels for bounding boxes within an image \citep{papandreou2014untangling, girshick2014rcnn}. Recently, there are several works that attemp to semantically segment an image with DCNN. \citet{girshick2014rcnn, hariharan2014simultaneous} take both bounding box proposals and masked regions as input to DCNN. The masked regions provide extra object shape informantion to the neural networks. These methods heavily depend on the region proposals \citep{arbelaez2014multiscale, Uijlings13}. 
%Note that second order pooling \citep{carreira2012semantic} also assigns labels to regions proposals \citep{carreira2012cpmc}; however, hand-crafted features are employed. 
\citet{farabet2013learning} apply DCNN to multi-resolution of the input image and employ a segmentation tree to smooth the prediction results. We notice that there are serveral concurrent works, which bear similarities to our proposed model. \citet{mostajabi2014feedforward} propose to combine the multi-scale cues extracted by DCNN (and some hand-crafted features) to label one superpixel. Similarly, their results depend on the superpixels, which may leak out the object boundaries, and the errors are difficult to recover. \citet{hariharan2014hypercolumns} propose to concatenate the computed inter-mediate feature maps within the DCNN for pixel classfication, and \citet{dai2014convolutional} propose to pool the inter-mediate feature maps by region proposals. Their models are two-step models, which depends on the accuracy of first step (\ie region proposals). On the other hand, our model is most similar to \citet{long2014fully, eigen2014predicting}, which directly apply DCNN to the whole image in sliding window fashion. The last fully connected layers within DCNN are replaced by convolutional layers. \citet{long2014fully} upsample and concatenate the scores from inter-mediate feature maps, while \citet{eigen2014predicting} refine the prediction result from coarse to fine by propagating the coarse results to another DCNN. 

{\bf{Combine Graphical Model and DCNN: }} The main difference between our model and other state-of-the-art models is the combination of graphical models and DCNN. Other works that are similar to ours include \citet{cogswell2014combining}, which employ CRF to propose diverse region proposals \citep{yadollahpour2013discriminative} and extract features via DCNN, and \citet{chen2014learning} which efficiently blend inference and learning to jointly train DCNN and CRF. Our current model employs piecewise training, and jointly training is our next goal.




